The GMRT archive atomic gas survey -- III. Comparative Study of Dark Matter Halos in Nearby Galaxies

The distribution of dark matter in the inner regions of galaxies poses a key challenge for small-scale {\Lambda}CDM cosmology. While cold dark matter simulations predict cuspy inner density profiles, observations of low surface brightness (LSB) and dwarf galaxies often favour cored profiles, an issue known as the cusp-core problem. We investigate this problem by comparing four dark matter halo profiles: NFW (cuspy), Einasto (intermediate), Burkert (cored), and pseudo-isothermal (pISO) (cored) in a pilot sample of $11$ galaxies from the GMRT archive atomic gas survey (GARCIA). We have performed mass modelling using Markov Chain Monte Carlo (MCMC) techniques, utilising rotation curves derived from robust 3D Kinematic modelling. Baryonic contributions from stars derived using stellar kinematics based on $3.6\mu\mathrm{m}$ or $r$-band photometry via Multi-Gaussian Expansion (MGE) combined with Jeans Anisotropic Model (JAM) and from gas, calculated directly from the gas surface density (HI + He) without assuming any predefined functional form, are included. Our mass modelling shows that all halo profiles provide statistically good fits, yielding consistent estimates of halo mass and stellar mass-to-light ratio. To validate our analysis, we examine the stellar-to-halo mass relation and find broad agreement with empirical models. Non-parametric density profiles derived from baryon-subtracted rotation curves show that NFW fits the inner regions best, while all profiles converge in the outskirts. Future studies with a larger sample from GARCIA will be helpful in refining this trend and addressing the cusp-core issue in greater depth.

==> Results_img/halo_table_two_tables.tex <==
%\begin{landscape}
%\usepackage{pdflscape}
\begin{adjustbox}{angle=90,center}
\onecolumn

{\scriptsize
\renewcommand{\arraystretch}{1.6} 

\begin{longtable}{l|ccc|ccc|ccc|ccc}
%
\caption{Best-fit $M_{200}$ (in $10^{11} M_\odot$), $M/L$ , and concentration parameter $c$ for the four DM halo profiles.} 
\label{MCMC-diffProf} \\
\toprule
\multirow{2}{*}{Galaxy} & \multicolumn{3}{c|}{NFW} & \multicolumn{3}{c|}{Einasto} & \multicolumn{3}{c|}{Burkert} & \multicolumn{3}{c}{pISO} \\
 & $M_{200}$ & $M/L$ & $c$ & $M_{200}$ & $M/L$ & $c$ & $M_{200}$ & $M/L$ & $c$ & $M_{200}$ & $M/L$ & $c$ \\
\midrule
\endhead
NGC0784 & $1.51^{+1.23}_{-3.00}$ & $0.62^{+0.18}_{-0.18}$ & $2.12^{+1.02}_{-2.57}$ & $1.83^{+1.50}_{-3.03}$ & $0.68^{+0.18}_{-0.17}$ & $3.05^{+0.79}_{-1.59}$ & $1.97^{+1.71}_{-3.24}$ & $0.75^{+0.17}_{-0.16}$ & $7.28^{+1.37}_{-2.43}$ & $1.59^{+1.10}_{-3.01}$ & $0.72^{+0.17}_{-0.17}$ & $17.54^{+4.47}_{-8.53}$ \\
NGC1156 & $1.36^{+1.16}_{-3.07}$ & $0.25^{+0.07}_{-0.07}$ & $1.79^{+0.95}_{-3.29}$ & $2.31^{+1.82}_{-3.06}$ & $0.30^{+0.06}_{-0.06}$ & $2.42^{+0.60}_{-1.08}$ & $2.62^{+2.02}_{-3.09}$ & $0.33^{+0.06}_{-0.06}$ & $6.20^{+0.99}_{-1.18}$ & $2.27^{+1.67}_{-3.07}$ & $0.32^{+0.06}_{-0.06}$ & $13.58^{+2.81}_{-4.67}$ \\
NGC3027 & $1.67^{+0.35}_{-0.52}$ & $0.65^{+0.19}_{-0.19}$ & $11.63^{+2.36}_{-2.61}$ & $0.86^{+0.17}_{-0.26}$ & $0.65^{+0.20}_{-0.20}$ & $11.11^{+1.61}_{-1.70}$ & $1.10^{+0.16}_{-0.20}$ & $0.72^{+0.19}_{-0.19}$ & $21.18^{+2.63}_{-2.86}$ & $4.54^{+0.68}_{-0.78}$ & $0.93^{+0.17}_{-0.18}$ & $50.12^{+7.63}_{-8.45}$ \\
NGC3359 & $5.19^{+0.39}_{-0.47}$ & $0.04^{+0.02}_{-0.04}$ & $8.70^{+0.85}_{-0.76}$ & $2.55^{+0.25}_{-0.32}$ & $0.18^{+0.05}_{-0.05}$ & $9.56^{+1.04}_{-1.16}$ & $3.18^{+0.25}_{-0.28}$ & $0.29^{+0.03}_{-0.03}$ & $16.60^{+1.64}_{-1.95}$ & $8.96^{+0.54}_{-0.60}$ & $0.30^{+0.03}_{-0.03}$ & $47.36^{+6.52}_{-7.57}$ \\
NGC4068 & $1.59^{+1.41}_{-3.09}$ & $0.51^{+0.16}_{-0.16}$ & $1.32^{+0.68}_{-2.15}$ & $2.37^{+1.89}_{-3.06}$ & $0.59^{+0.15}_{-0.16}$ & $2.56^{+0.51}_{-0.83}$ & $2.72^{+2.09}_{-3.05}$ & $0.64^{+0.15}_{-0.15}$ & $7.20^{+0.95}_{-1.04}$ & $2.45^{+1.90}_{-3.10}$ & $0.63^{+0.15}_{-0.15}$ & $15.89^{+2.64}_{-3.58}$ \\
NGC4861 & $3.73^{+1.93}_{-2.71}$ & $0.09^{+0.06}_{-0.09}$ & $1.82^{+0.41}_{-0.67}$ & $3.80^{+2.10}_{-2.83}$ & $0.21^{+0.10}_{-0.11}$ & $3.07^{+0.31}_{-0.51}$ & $3.40^{+1.98}_{-2.84}$ & $0.30^{+0.10}_{-0.10}$ & $7.91^{+0.42}_{-0.58}$ & $3.92^{+1.85}_{-2.66}$ & $0.29^{+0.10}_{-0.10}$ & $17.76^{+1.31}_{-1.96}$ \\
NGC7292 & $2.60^{+0.96}_{-1.89}$ & $2.22^{+0.88}_{-0.88}$ & $12.26^{+2.95}_{-3.81}$ & $1.00^{+0.45}_{-1.35}$ & $2.84^{+0.98}_{-0.97}$ & $12.43^{+2.97}_{-3.68}$ & $1.30^{+0.39}_{-0.89}$ & $3.77^{+0.84}_{-0.87}$ & $23.97^{+3.86}_{-4.29}$ & $7.82^{+1.59}_{-1.94}$ & $4.56^{+0.72}_{-0.75}$ & $58.23^{+6.88}_{-7.77}$ \\
NGC7497 & $2.36^{+0.42}_{-0.73}$ & $0.58^{+0.13}_{-0.13}$ & $12.05^{+3.30}_{-3.49}$ & $1.30^{+0.29}_{-0.59}$ & $0.67^{+0.13}_{-0.13}$ & $10.23^{+2.42}_{-2.53}$ & $1.61^{+0.28}_{-0.48}$ & $0.76^{+0.11}_{-0.12}$ & $18.44^{+4.32}_{-4.18}$ & $5.69^{+0.88}_{-1.06}$ & $0.85^{+0.08}_{-0.09}$ & $42.96^{+9.30}_{-9.95}$ \\
NGC7610 & $3.59^{+1.21}_{-2.23}$ & $3.10^{+0.56}_{-0.43}$ & $5.45^{+2.02}_{-4.04}$ & $4.21^{+1.77}_{-2.52}$ & $3.59^{+0.33}_{-0.31}$ & $3.96^{+0.84}_{-1.30}$ & $3.95^{+1.38}_{-2.21}$ & $3.78^{+0.29}_{-0.28}$ & $7.44^{+1.19}_{-1.65}$ & $6.33^{+1.65}_{-2.08}$ & $3.77^{+0.28}_{-0.28}$ & $17.83^{+3.78}_{-5.21}$ \\
NGC7741 & $0.43^{+0.08}_{-0.10}$ & $0.99^{+0.14}_{-0.14}$ & $17.68^{+3.79}_{-3.93}$ & $0.19^{+0.03}_{-0.03}$ & $0.75^{+0.17}_{-0.17}$ & $21.35^{+3.48}_{-3.51}$ & $0.32^{+0.05}_{-0.06}$ & $1.00^{+0.15}_{-0.15}$ & $28.56^{+4.93}_{-5.19}$ & $1.32^{+0.32}_{-0.39}$ & $1.28^{+0.11}_{-0.11}$ & $43.78^{+9.28}_{-10.00}$ \\
NGC7800 & $5.75^{+1.17}_{-1.62}$ & $0.23^{+0.13}_{-0.15}$ & $7.47^{+1.10}_{-1.26}$ & $3.06^{+0.68}_{-1.03}$ & $0.33^{+0.15}_{-0.16}$ & $8.06^{+0.95}_{-1.02}$ & $2.85^{+0.37}_{-0.49}$ & $0.45^{+0.15}_{-0.15}$ & $17.24^{+1.63}_{-1.79}$ & $10.44^{+1.01}_{-1.18}$ & $0.48^{+0.14}_{-0.14}$ & $46.23^{+5.18}_{-5.91}$ \\
\bottomrule
\end{longtable}
}
\end{adjustbox}
%\end{scriptsize}
\twocolumn
%\end{landscape}

%\onecolumn
\begin{scriptsize}
\begin{longtable}{lcccc}
\caption{Reduced $\chi^2$ values for the four DM halo models.} \label{tab:long_chisq} \\
\toprule
Galaxy & NFW & Einasto & Burkert & pISO \\
\midrule
\endfirsthead
\caption[]{(continued)} \\
\toprule
Galaxy & NFW & Einasto & Burkert & pISO \\
\midrule
\endhead
NGC0784 & 0.368 & 0.278 & 0.324 & 0.295 \\
NGC1156 & 0.193 & 0.207 & 0.274 & 0.237 \\
NGC3027 & 0.061 & 0.106 & 0.205 & 0.416 \\
NGC3359 & 1.503 & 0.317 & 0.221 & 0.993 \\
NGC4068 & 0.096 & 0.081 & 0.139 & 0.125 \\
NGC4861 & 2.734 & 2.153 & 2.017 & 2.025 \\
NGC7292 & 0.885 & 0.721 & 1.225 & 2.414 \\
NGC7497 & 0.630 & 0.978 & 1.583 & 1.406 \\
NGC7610 & 5.246 & 4.945 & 4.441 & 4.695 \\
NGC7741 & 6.869 & 4.999 & 5.853 & 8.022 \\
NGC7800 & 1.495 & 1.015 & 0.434 & 0.930 \\
\bottomrule
\end{longtable}
\end{scriptsize}
%\twocolumn
